DiffFit: Unlocking Transferability of Large Diffusion Models via Simple Parameter-Efficient Fine-Tuning

Diffusion models have proven to be highly effective in generating high-quality images. However, adapting large pre-trained diffusion models to new domains remains an open challenge, which is critical for real-world applications. This paper proposes DiffFit, a parameter-efficient strategy to fine-tune large pre-trained diffusion models that enable fast adaptation to new domains. DiffFit is embarrassingly simple that only fine-tunes the bias term and newly-added scaling factors in specific layers, yet resulting in significant training speed-up and reduced model storage costs. Compared with full fine-tuning, DiffFit achieves 2$\times$ training speed-up and only needs to store approximately 0.12\% of the total model parameters. Intuitive theoretical analysis has been provided to justify the efficacy of scaling factors on fast adaptation. On 8 downstream datasets, DiffFit achieves superior or competitive performances compared to the full fine-tuning while being more efficient. Remarkably, we show that DiffFit can adapt a pre-trained low-resolution generative model to a high-resolution one by adding minimal cost. Among diffusion-based methods, DiffFit sets a new state-of-the-art FID of 3.02 on ImageNet 512$\times$512 benchmark by fine-tuning only 25 epochs from a public pre-trained ImageNet 256$\times$256 checkpoint while being 30$\times$ more training efficient than the closest competitor.

==> tabs/finetune_strategy.tex <==
\begin{table}[t]
% \vspace{-.5em}
\centering
\begin{tabular}{l|cccc}
\toprule
method & epoch & \#params & FID $\downarrow$ \\
\midrule
Scratch  & 200 & &  14.11  \\
Full Fine-tune  & 80 & &  10.46  \\
Linear  & 80 & &  20.37  \\
BitFit  & 80 & &  9.17  \\
\rowcolor{gray!10}
~~+Scale  & 80 & &  \textbf{8.19}  \\
\bottomrule
\end{tabular}
\caption{ \textbf{Comparison of fine-tuning strategies. }
} 
\label{tab:ab4} \vspace{-1em}
\end{table}
